The Fourth Monocular Depth Estimation Challenge

This paper presents the results of the fourth edition of the Monocular Depth Estimation Challenge (MDEC), which focuses on zero-shot generalization to the SYNS-Patches benchmark, a dataset featuring challenging environments in both natural and indoor settings. In this edition, we revised the evaluation protocol to use least-squares alignment with two degrees of freedom to support disparity and affine-invariant predictions. We also revised the baselines and included popular off-the-shelf methods: Depth Anything v2 and Marigold. The challenge received a total of 24 submissions that outperformed the baselines on the test set; 10 of these included a report describing their approach, with most leading methods relying on affine-invariant predictions. The challenge winners improved the 3D F-Score over the previous edition's best result, raising it from 22.58% to 23.05%.

==> Figures/depth.tex <==
% SYNS-Patches Depth Visualizations

\tiny

\def\first{0639}
\def\nums{0389,0039,0621,0682,0599,0745,0763}
\def\dataset{SynsDepth2025}

\def\methods{
    img/
    ,gt/GT
    ,mazhenxin/HRI
    ,previous/PICO-MR
    ,lavreniuk/Lavreniuk
    ,guanhaining/Mach-Calib
    ,easymono/EasyMono
    ,Louzq/Insta360-Percep
    ,zihanqin/HIT-AIIA   
    ,ppzu2/Robot02-vRobotit
    ,rmf3mc/ViGIR\_LAB
    ,yangtuananh/HCMUS-DepthFusion
    ,al/ReadingLS
}



\def\w{0.122\linewidth}

\foreach \method/\label in \methods{%
    \begin{tikzpicture}[every node/.style={inner sep=0,outer sep=0,anchor=south west}]
        \node (image) at (0, 0) {\includegraphics[width=\w]{\dataset/\first_\method.jpg}};
        \begin{scope}[x={(image.south east)},y={(image.north west)}]
            \draw (0.01, 0.01) node {\color{white}{\textbf{\label}}};
        \end{scope}
    \end{tikzpicture}
    %
    \foreach \num in \nums{%
        \includegraphics[width=\w]{\dataset/\num_\method.jpg}
    } \\
}


\vspace{-0.2cm}
\mycaption{Qualitatives on \acl{syns}}{%
Best viewed in color and zoomed in. Methods are ranked based on their F-Score in \tbl{res:results}. 

}


==> Figures/syns.tex <==
% SYNS-Patches Sample Images



\foreach \img in {img, gt}{%
    \foreach \num in {0012, 0120, 0730}{%
        \includegraphics[width=0.33\linewidth]{Syns_2024/\num_\img.jpeg}%
    }\\\vspace{-1pt}%
}


\mycaption{\acl{syns} Dataset}{%
The dataset contains samples from diverse scenes, including complex urban, natural, and indoor spaces. 
High-quality ground-truth depth measurements cover $\sim$78.20\% of pixels; edges and object boundary annotations are also available.
}


==> Tables/results.tex <==
% SYNS-Patches Results

% \footnotesize

% \def\n{9}

% \mycaption{\acl{syns} Results}{%
% %We provide metrics across the whole dataset and per scene-category. 
% %As expected, supervised methods generally outperform self-supervised ones. 
% %The largest gap can be found in Indoor scenes, self-supervised methods were trained exclusively on automotive data. 
% %Teams~\team{4} \& \team{5} outperformed the challenge baseline~\cite{Spencer2022} by incorporating more advanced network architectures.
% We provide metrics across the whole test split of the dataset. Top-performing entries generally leverage the pre-trained Depth Anything \cite{Yang2024} model. Only a few methods use self-supervised losses or proxy depth labels.
% }\vspace{-0.3cm}

% \begin{tabular}{@{}rrrrrrrrrrr@{}}
% \toprule
%                                            &            & Train & Rank &        F\up & F-Edges\up &     MAE\down &    RMSE\down &      AbsRel\down & Acc-Edges\down & Comp-Edges\down \\ 
% \midrule           
            
%            &  \team{1} & \train{1} &  \best{1} & \best{23.72} & \nbest{11.01} & \nbest{3.78} & \nbest{6.61} & 21.24 & 3.90 & 4.45 \\ 
%            &  \team{2} & \train{2} & \nbest{2} & \nbest{23.25} & 10.78 & 3.87 & 6.70 & 21.70 & 3.59 & 9.86 \\ 
%            &  \team{3} & \train{3} &         3 & 22.79 & \best{11.52} & 5.21 & 9.23 & 28.86 & 4.15 & \nbest{0.90} \\ 
%            &  \team{4} & \train{4} &         4 & 20.87 & 10.92 & \best{3.71} & \best{6.53} & \best{19.02} & 2.88 & 6.77 \\ 
%            &  \team{5} & \train{5} &         5 & 20.77 & 9.96 & 4.33 & 7.83 & 27.80 & 3.45 & 13.25 \\ 
%            &  \team{6} & \train{6} &         6 & 20.42 & 10.19 &	4.41 &	7.89 &	23.94 &	3.61 &	5.80 \\ 
%            & \team{7} & \train{7} &           7 & 19.07 & 9.92 & 4.53 & 7.96 & 23.27 & 3.26 & 8.00 \\
%            &  \team{8} & \train{8} &         8 & 18.60 &	9.43 &	3.92 &	7.16 &	\nbest{20.12} &	2.89 &	15.65 \\ 
%            &  \team{9} & \train{9} &        9 & 17.83 &	9.14 &	4.11 &	7.73 &	21.23 &	2.95 &	17.81 \\
%            &  \team{10} & \train{10} &        10 & 17.81 &	9.75 &	5.04 &	8.92 &	24.01 &	3.16 &	14.16 \\
%            &  \team{11} & \train{11} &        11 & 17.57 &	9.13 &	4.28 &	8.36 &	23.35 &	3.18 &	20.66 \\
%            &  \team{12} & \train{12} &        12 & 16.91 &	9.07 &	4.14 &	7.35 &	22.05 &	3.24 &	18.52 \\
%            &  \team{13} & \train{13} &        13 & 16.71 &	9.25 &	5.48 &	11.05 &	34.20 &	\best{2.57} &	18.04 \\
%            &  \team{14} & \train{14} &        14 & 16.45 &	8.89 &	5.29 &	10.53 &	33.67 &	\nbest{2.60} &	18.73 \\
%            &  \team{15} & \train{15} &        15 & 15.92 &	9.17 &	8.25 &	13.88 &	43.88 &	4.11 &	\best{0.74} \\
%            &  \team{16} & \train{16} &        16 & 14.81 &	8.14 &	5.01 &	8.94 &	29.39 &	3.28 &	30.28 \\
%            &  \team{0} & \train{0} &        17 & 13.72 &	7.76 &	5.56 &	9.72 &	32.04 &	3.97 &	21.63 \\
%            &  \team{17} & \train{17} &        18 & 13.71 &	7.55 &	5.49 &	9.44 &	30.74 &	3.61 &	18.36 \\
%            &  \team{18} & \train{18} &        19 & 11.90 &	8.08 &	6.33 &	10.89 &	30.46 &	2.99 &	33.63 \\
%            &  \team{19} & \train{19} &        20 & 11.04 & 7.09 & 8.76 & 15.86 & 63.32 & 3.22 & 40.61 \\

%            % &  \team{1} & \train{1} &  \best{1} & 23.7210 & 11.0130 & 3.7787 & 6.6115 & 21.2386 & 3.8974 & 4.4517 \\ 
%            % &  \team{2} & \train{3} & \nbest{2} & 23.2499 & 10.7783 & 3.8725 & 6.7038 & 21.6987 & 3.5911 & 9.8569 \\ 
%            % &  \team{3} & \train{3} &         3 & 22.7924 & 11.5192 & 5.2061 & 9.2339 & 28.8613 & 4.1541 & 0.8980 \\ 
%            % &  \team{4} & \train{5} &         4 & 20.8658 & 10.9224 & 3.7086 & 6.5308 & 19.0214 & 2.8835 & 6.7700 \\ 
%            % &  \team{5} & \train{6} &         5 & 20.7673 & 9.9617 & 4.3302 & 7.8348 & 27.7973 & 3.4458 & 13.2527 \\ 
%            % &  \team{6} & \train{8} &         6 & 20.4244 & 10.1868 &	4.4079 &	7.8909 &	23.9416 &	3.6105 &	5.7953 \\ 
%            % &  \team{7} & \train{4} &         7 & 18.5956 &	9.4273 &	3.9224 &	7.1649 &	20.1185 &	2.8921 &	15.6460 \\ 
%            % &  \team{8} & \train{7} &         8 & 18.4475 &	9.7061 &	4.7358 &	8.6001 &	25.6061 &	3.3700 &	6.6398 \\
%            % &  \team{10} & \train{8} &        10 & 17.8328 &	9.1387 &	4.1147 &	7.7332 &	21.2310 &	2.9465 &	17.8145 \\
%            % &  \team{11} & \train{8} &        11 & 17.8121 &	9.7525 &	5.0386 &	8.9196 &	24.0101 &	3.1615 &	14.1550 \\
%            % &  \team{12} & \train{8} &        12 & 17.5704 &	9.1273 &	4.2759 &	8.3635 &	23.3455 &	3.1765 &	20.6621 \\
%            % &  \team{13} & \train{8} &        13 & 16.9120 &	9.0666 &	4.1357 &	7.3481 &	22.0509 &	3.2377 &	18.5220 \\
%            % &  \team{14} & \train{8} &        14 & 16.7148 &	9.2525 &	5.4767 &	11.0510 &	34.2035 &	2.5703 &	18.0436 \\
%            % &  \team{15} & \train{8} &        15 & 16.4478 &	8.8896 &	5.2907 &	10.5310 &	33.6741 &	2.5965 &	18.7283 \\
%            % &  \team{16} & \train{8} &        16 & 15.9223 &	9.1679 &	8.2542 &	13.8783 &	43.8823 &	4.1054 &	0.7403 \\
%            % &  \team{17} & \train{8} &        17 & 14.8093 &	8.1357 &	5.0099 &	8.9448 &	29.3938 &	3.2837 &	30.2778 \\
%            % &  \team{0} & \train{0} &        18 & 13.7211 &	7.7630 &	5.5645 &	9.7169 &	32.0420 &	3.9712 &	21.6256 \\
%            % &  \team{18} & \train{8} &        19 & 13.7089 &	7.5505 &	5.4867 &	9.4419 &	30.7377 &	3.6072 &	18.3600 \\
%            % &  \team{19} & \train{8} &        20 & 11.8998 &	8.0770 &	6.3256 &	10.8861 &	30.4607 &	2.9862 &	33.6279 \\
%            %&  \team{20} & \train{8} &        21 & 11.0444 & 7.0866 & 8.7645 & 15.8637 & 63.3160 & 3.2209 & 40.6098 \\
% \bottomrule
% \end{tabular}

% \emph{
% \textbf{M}=Monocular -- \textbf{S}=Stereo -- \textbf{D*}=Proxy Depth -- \textbf{D}=Ground-truth Depth -- \textbf{$\dagger$}=Pre-trained Depth Anything model
% }







\footnotesize

\def\n{9}
\mycaption{\acl{syns} Results}{%
%We provide metrics across the whole dataset and per scene-category. 
%As expected, supervised methods generally outperform self-supervised ones. 
%The largest gap can be found in Indoor scenes, self-supervised methods were trained exclusively on automotive data. 
%Teams~\team{4} \& \team{5} outperformed the challenge baseline~\cite{Spencer2022} by incorporating more advanced network architectures.
We provide metrics across the whole test split of the dataset. 
%Top-performing entries generally employ the affine-invariant prediction type ($\mathcal{A}$). 
%Only a few methods use self-supervised losses or proxy depth labels.
}\vspace{-0.3cm}
\scalebox{0.82}{
\begin{tabular}{@{}rlrrrrrrrrrrrr@{}}
\toprule
                                           & Team       &  & Rank &        F\up & F-Edges\up &     MAE\down &    RMSE\down &      AbsRel\down & Acc-Edges\down & Comp-Edges\down & $\delta < 1.25$\up & $\delta < 1.25^2$\up & $\delta < 1.25^3$\up \\ 
\midrule           
            
           $\mathcal{A}$ &  \team{1} & %\train{1} 
           & 1 & \fst 23.05  & \snd 9.37  & \fst 3.19  & \fst 5.64  & \snd 21.17  & 3.30 & \snd 6.77 & \snd 77.54  & \snd 91.79  & \trd 95.78   \\ 
           & \textcolor{gray}{\textit{Anonymous}} & & 2 & \snd 22.95  & 9.21  & 3.44  & 6.48  & 24.65 & 3.27 & \fst 6.59  & \trd 76.17  & 90.33  & 94.73 \\
           \rowcolor{Asectioncolor}
           & \bf PICO-MR \cite{Spencer_2024_CVPR} & & %3 
           - & 22.58  & 8.26  & 3.41  & 5.89  & 22.02  & 4.02  & 11.28  & 76.18  &  90.95  & 95.44  \\
           $\mathcal{A}$ & \team{2} & & 3 & \trd 20.81  & 9.12  & \trd 3.40  & \trd 5.77  & \fst 20.48  & 3.20  & \trd 7.27  & 75.33  & \trd 91.33  & \fst 95.97 \\
           $\mathcal{A}$ & \team{3} & & 4 & 20.69  & 8.75  & 3.63  & 6.78  & 23.36  & 3.22  & 13.96  & 74.31  & 90.44  & 95.12  \\
           & \textcolor{gray}{\textit{Anonymous}} & & 5 & 20.50  & 8.63  & 3.68  & 7.07  & 23.96  & 3.17  & 13.66  & 74.00  & 90.32  & 95.01 \\
           $\mathcal{A}$ & \team{4} & & 6 & 20.24  & 7.30  & 3.43  & 5.91  & 22.47  & 3.91  & 20.98  & 74.73  & 90.55  & 95.24 \\
           $\mathcal{A}$ & \team{5} & & 7 & 19.41  & 8.98  & \snd 3.25 & \snd 5.73  & \trd 21.29  & \fst 2.75  & 15.54  & \fst 77.91  & \fst 92.03  & \snd 95.91 \\ 
           & \textcolor{gray}{\textit{Anonymous}} & & 8 & 18.85  & 8.27  & 4.06  & 7.06  & 26.35  & 3.11  & 13.75  & 67.57  & 87.98  & 94.18 \\ 
           $\mathcal{A}$ & \team{6} & & 9 & 18.53  & \fst 9.74  & 3.83  & 6.29  & 23.96  & \trd 3.06 & 9.90  & 69.12  & 88.49  & 94.31 \\ 
           & \textcolor{gray}{\textit{Anonymous}} & & 10 & 18.16  & 6.32  & 3.57  & 6.13  & 24.07  & 4.51  & 15.75  & 71.62  & 89.12  & 94.74 \\ 
           \multirow{3}{*}{$\dagger$ $\left\{ \vphantom{\begin{tabular}{c}3\\3\\3\end{tabular}}\right.$} & \textcolor{gray}{\textit{Anonymous}} & & 11 & 17.46  & \trd 9.35  & 4.43  & 7.30  & 29.19  & 3.27  & 17.69 & 65.64  & 86.45  & 93.09 \\ 
           & \textcolor{gray}{\textit{Anonymous}} & & 12 & 17.46  & \trd 9.35  & 4.43  & 7.30  & 29.19  & 3.27  & 17.69  & 65.64  & 86.45  & 93.09 \\
           & \textcolor{gray}{\textit{Anonymous}} & & 13 & 17.45  & \trd 9.35  & 4.43  & 7.30  & 29.20  & 3.27  & 17.69  & 65.64  & 86.46  & 93.10 \\ 
           $\mathcal{A}$ & \team{7} & & 14 & 17.25  & 8.27  & 3.90  & 6.54  & 23.64  & 3.07  & 22.85  & 71.07  & 89.38  & 94.80 \\ 
           \multirow{2}{*}{* \bf $\left\{ \vphantom{\begin{tabular}{c}2\\2\end{tabular}}\right.$} & \textcolor{gray}{\textit{Anonymous}} & & 15 & 17.01  & 9.20  & 4.44  & 7.34  & 29.42  & 3.25  & 18.55  & 65.72  & 86.67  & 93.35 \\ 
           & \textcolor{gray}{\textit{Anonymous}} & & 16 & 17.01  & 9.20  & 4.44  & 7.34  & 29.42  & 3.25 & 18.55  & 65.72  & 86.67  & 93.35 \\ 
           \rowcolor{Dsectioncolor}
           $\mathcal{A}$ & \bf Marigold \cite{ke2024repurposing} & & %18 
           - & 17.01  & 9.19  & 4.44  & 7.34  & 29.42  & 3.25 & 18.56  & 65.72  & 86.67  & 93.35 \\ 
           & \textcolor{gray}{\textit{Anonymous}} & & 17 & 16.79  & 9.10  & 4.51  & 7.44  & 30.10  & 3.32  & 17.65  & 65.24  & 86.22  & 93.05 \\ 
           & \textcolor{gray}{\textit{Anonymous}} & & 18 & 16.67  & 7.49  & 4.01  & 6.92  & 26.34  & 3.07  & 26.32  & 68.17  & 88.47  & 94.42 \\ 
           & \textcolor{gray}{\textit{Anonymous}} & & 19 & 16.47  & 8.99  & 4.74  & 7.71  & 30.93  & 3.26  & 18.75  & 62.26  & 84.27  & 91.90\\ 
           & \team{8} & & 20 & 16.25  & 8.54  & 5.37  & 9.00 & 43.72  & 3.29  & 14.15  & 61.99  & 82.89  & 90.46 \\ 
           $\mathcal{A}$ & \textcolor{gray}{\textit{Anonymous}} & & 21 & 15.31  & 8.46  & 4.62  & 7.46  & 30.63  & 3.42  & 15.59  & 62.41  & 84.89  & 92.43 \\ 
           & \textcolor{gray}{\textit{Anonymous}} & & 22 & 15.03  & 7.64  & 5.48  & 9.29  & 38.59  & 3.70  & 20.33  & 58.82  & 81.79  & 90.85\\ 
           \rowcolor{Dsectioncolor}
           & \bf Depth Anything v2 \cite{Yang2024v2} & & %25 
            - & 14.34  & 6.72  & 4.84  & 9.13  & 33.57  & \snd 2.99  & 35.54  & 66.34  & 86.02  & 92.44 \\ 
           $\mathcal{A}$ & \team{9} & & 23 & 14.20  & 7.81  & 4.90  & 7.96  & 33.55  & 3.32  & 17.66  & 61.09  & 83.90  & 92.21 \\ 
           & \team{10} & & 24 & 13.52  & 6.60  & 4.56  & 7.90 & 30.15  & 3.14  & 35.94  & 65.34  & 86.55  & 93.46  \\ 

           % &  \team{1} & \train{1} &  \best{1} & 23.7210 & 11.0130 & 3.7787 & 6.6115 & 21.2386 & 3.8974 & 4.4517 \\ 
           % &  \team{2} & \train{3} & \nbest{2} & 23.2499 & 10.7783 & 3.8725 & 6.7038 & 21.6987 & 3.5911 & 9.8569 \\ 
           % &  \team{3} & \train{3} &         3 & 22.7924 & 11.5192 & 5.2061 & 9.2339 & 28.8613 & 4.1541 & 0.8980 \\ 
           % &  \team{4} & \train{5} &         4 & 20.8658 & 10.9224 & 3.7086 & 6.5308 & 19.0214 & 2.8835 & 6.7700 \\ 
           % &  \team{5} & \train{6} &         5 & 20.7673 & 9.9617 & 4.3302 & 7.8348 & 27.7973 & 3.4458 & 13.2527 \\ 
           % &  \team{6} & \train{8} &         6 & 20.4244 & 10.1868 &	4.4079 &	7.8909 &	23.9416 &	3.6105 &	5.7953 \\ 
           % &  \team{7} & \train{4} &         7 & 18.5956 &	9.4273 &	3.9224 &	7.1649 &	20.1185 &	2.8921 &	15.6460 \\ 
           % &  \team{8} & \train{7} &         8 & 18.4475 &	9.7061 &	4.7358 &	8.6001 &	25.6061 &	3.3700 &	6.6398 \\
           % &  \team{10} & \train{8} &        10 & 17.8328 &	9.1387 &	4.1147 &	7.7332 &	21.2310 &	2.9465 &	17.8145 \\
           % &  \team{11} & \train{8} &        11 & 17.8121 &	9.7525 &	5.0386 &	8.9196 &	24.0101 &	3.1615 &	14.1550 \\
           % &  \team{12} & \train{8} &        12 & 17.5704 &	9.1273 &	4.2759 &	8.3635 &	23.3455 &	3.1765 &	20.6621 \\
           % &  \team{13} & \train{8} &        13 & 16.9120 &	9.0666 &	4.1357 &	7.3481 &	22.0509 &	3.2377 &	18.5220 \\
           % &  \team{14} & \train{8} &        14 & 16.7148 &	9.2525 &	5.4767 &	11.0510 &	34.2035 &	2.5703 &	18.0436 \\
           % &  \team{15} & \train{8} &        15 & 16.4478 &	8.8896 &	5.2907 &	10.5310 &	33.6741 &	2.5965 &	18.7283 \\
           % &  \team{16} & \train{8} &        16 & 15.9223 &	9.1679 &	8.2542 &	13.8783 &	43.8823 &	4.1054 &	0.7403 \\
           % &  \team{17} & \train{8} &        17 & 14.8093 &	8.1357 &	5.0099 &	8.9448 &	29.3938 &	3.2837 &	30.2778 \\
           % &  \team{0} & \train{0} &        18 & 13.7211 &	7.7630 &	5.5645 &	9.7169 &	32.0420 &	3.9712 &	21.6256 \\
           % &  \team{18} & \train{8} &        19 & 13.7089 &	7.5505 &	5.4867 &	9.4419 &	30.7377 &	3.6072 &	18.3600 \\
           % &  \team{19} & \train{8} &        20 & 11.8998 &	8.0770 &	6.3256 &	10.8861 &	30.4607 &	2.9862 &	33.6279 \\
           %&  \team{20} & \train{8} &        21 & 11.0444 & 7.0866 & 8.7645 & 15.8637 & 63.3160 & 3.2209 & 40.6098 \\
\bottomrule
\end{tabular}}
\emph{Legend: 
\colorbox{Dsectioncolor}{\textbf{Baselines}}; \colorbox{Asectioncolor}{\textbf{3rd MDEC winning team}}; {$\dagger$ -- likely the same method}; 
{* -- likely minor variations of Marigold}; 
{$\mathcal{A}$ -- affine-invariant predictions; \hspace{0.5cm} for each metric we highlight \colorbox{firstcolor}{\textbf{absolute best}}, \colorbox{secondcolor}{second best}, \colorbox{thirdcolor}{third best}}
%\textbf{M}=Monocular -- \textbf{S}=Stereo -- \textbf{D*}=Proxy Depth -- \textbf{D}=Ground-truth Depth -- \textbf{$\dagger$}=Pre-trained Depth Anything model
}\vspace{-0.2cm}


==> Tables/results_2023.tex <==
% SYNS-Patches Results

\footnotesize

\def\n{9}

\mycaption{\acl{syns} Results}{%
We provide metrics across the whole dataset and per scene-category. 
As expected, supervised methods generally outperform self-supervised ones. 
The largest gap can be found in Indoor scenes, self-supervised methods were trained exclusively on automotive data. 
Teams~\team{4} \& \team{5} outperformed the challenge baseline~\cite{Spencer2022} by incorporating more advanced network architectures.
}

\begin{tabular}{@{}lllllllllll@{}}
\toprule
                                           &            & Train & Rank &        F\up & F-Edges\up &     MAE\down &    RMSE\down &      AbsRel\down & Acc-Edges\down & Comp-Edges\down \\ 
\midrule           
            
            \multirow{\n}*{\emph{Overall}} &  \team{1} & \train{1} &  \best{1} &  \best{17.51} &         8.80 &  \best{4.52} &         8.72 &  \best{24.32} &         3.22 &         21.65 \\ 
                                           &  \team{2} & \train{3} & \nbest{2} & \nbest{16.94} &  \best{9.63} & \nbest{4.71} &  \best{8.00} &         25.35 &         3.56 &         19.95 \\ 
                                           &  \team{3} & \train{3} &         3 &         16.70 & \nbest{9.36} &         4.91 &         8.63 & \nbest{24.33} &  \best{3.02} &         18.07 \\ 
                                           &  \team{5} & \train{5} &         4 &         16.00 &         8.49 &         5.08 &         8.96 &         28.46 &         3.74 &  \best{11.32} \\ 
                                           &  \team{6} & \train{6} &         5 &         14.71 &         8.13 &         5.17 &         8.97 &         29.43 &         3.75 & \nbest{17.29} \\ 
                                           &  \team{0} & \train{0} &         6 &         13.72 &         7.76 &         5.56 &         9.72 &         32.04 &         3.97 &         21.63 \\ 
                                        %   &  \team{9} & \train{9} &         7 &         13.23 &         8.26 &         5.18 &         8.76 &         28.03 & \nbest{3.07} &         29.96 \\ 
                                           &  \team{4} & \train{4} &         7 &         12.77 &         7.68 &         5.17 &         8.83 &         29.92 &         3.56 &         35.26 \\ 
                                           &  \team{7} & \train{7} &         8 &         12.44 &         7.49 &         5.05 & \nbest{8.59} &         28.99 & \nbest{3.10} &         38.93 \\ 
                                           &  \team{8} & \train{8} &        9 &         11.29 &         7.18 &         5.81 &         9.58 &         32.82 &         3.47 &         43.38 \\ 
                                        %   &\team{10} & \train{10} &        11 &          9.99 &         6.74 &         5.95 &         9.69 &         34.49 &         3.51 &         47.95 \\ 
\midrule
      \multirow{\n}*{\emph{Outdoor-Urban}} &  \team{1} & \train{1} &  \best{1} &  \best{16.41} &         7.37 &  \best{3.81} &         7.82 &  \best{21.85} &         2.91 &         24.36 \\ 
                                           &  \team{5} & \train{5} &         4 & \nbest{16.28} &         7.27 &         4.49 &         7.98 &         26.18 &         3.67 &  \best{13.11} \\ 
                                           &  \team{6} & \train{6} &         5 &         15.21 &         6.80 &         4.60 &         8.00 &         27.55 &         3.73 &         16.26 \\ 
                                           &  \team{2} & \train{3} & \nbest{2} &         15.10 &  \best{8.48} & \nbest{4.03} &  \best{6.90} &         23.67 &         3.36 &         19.13 \\ 
                                           &  \team{3} & \train{3} &         3 &         15.01 & \nbest{7.79} &         4.26 &         7.70 & \nbest{22.88} & \nbest{2.87} & \nbest{15.73} \\ 
                                           &  \team{0} & \train{0} &         6 &         14.09 &         6.48 &         4.77 &         8.43 &         29.10 &         3.89 &         22.75 \\ 
                                           &  \team{4} & \train{4} &         7 &         12.90 &         5.92 &         4.49 &         7.80 &         27.44 &         3.26 &         35.36 \\ 
                                        %   &  \team{9} & \train{9} &         7 &         12.53 &         6.43 &         4.61 &         7.93 &         26.28 &  \best{2.82} &         27.07 \\ 
                                           &  \team{7} & \train{7} &         8 &         12.52 &         5.89 &         4.37 & \nbest{7.62} &         26.46 &  \best{2.83} &         40.33 \\ 
                                           &  \team{8} & \train{8} &         9 &         11.31 &         5.73 &         5.14 &         8.69 &         30.64 &         3.13 &         40.15 \\ 
                                        %   &\team{10} & \train{10} &        11 &          9.95 &         5.18 &         5.20 &         8.73 &         32.12 &         3.15 &         43.54 \\ 
\midrule   
    \multirow{\n}*{\emph{Outdoor-Natural}} &  \team{2} & \train{3} & \nbest{2} &  \best{14.90} & \nbest{6.75} & \nbest{6.26} &  \best{10.47} &         28.40 &         3.54 &         14.44 \\ 
                                           &  \team{3} & \train{3} &         3 & \nbest{14.66} &  \best{6.79} &         6.35 &         10.86 & \nbest{27.09} &  \best{3.08} &         19.73 \\ 
                                           &  \team{5} & \train{5} &         4 &         14.43 &         6.02 &         6.51 &         11.43 &         30.57 &         3.59 &   \best{9.44} \\ 
                                           &  \team{1} & \train{1} &  \best{1} &         14.31 &         6.07 &  \best{5.97} & \nbest{10.81} &  \best{26.48} &         3.45 &         17.75 \\ 
                                           &  \team{6} & \train{6} &         5 &         12.89 &         5.74 &         6.77 &         11.62 &         32.57 &         3.68 & \nbest{13.97} \\ 
                                           &  \team{0} & \train{0} &         6 &         12.10 &         5.32 &         7.46 &         12.86 &         36.89 &         3.84 &         18.35 \\ 
                                           &  \team{4} & \train{4} &         7 &         11.54 &         6.03 &         6.87 &         11.52 &         33.66 &         3.36 &         32.47 \\ 
                                        %   &  \team{9} & \train{9} &         7 &         11.28 &         6.12 &         6.75 &         11.02 &         32.03 & \nbest{3.09} &         28.65 \\ 
                                           &  \team{7} & \train{7} &         8 &         10.98 &         5.38 &         6.66 &         11.13 &         32.19 & \nbest{3.13} &         36.01 \\ 
                                           &  \team{8} & \train{8} &         9 &          9.26 &         4.92 &         7.69 &         12.22 &         38.14 &         3.36 &         42.92 \\ 
                                        %   &\team{10} & \train{10} &        11 &          7.73 &         4.33 &         7.91 &         12.41 &         40.51 &         3.39 &         47.33 \\ 
\midrule   
\multirow{\n}*{\emph{Outdoor-Agriculture}} &  \team{1} & \train{1} &  \best{1} &  \best{16.36} &         5.24 &  \best{5.17} &        10.13 &         29.07 &         3.43 &         18.84 \\ 
                                           &  \team{2} & \train{3} & \nbest{2} & \nbest{15.58} &  \best{6.40} & \nbest{5.25} &  \best{9.09} & \nbest{27.45} &         3.64 &         18.30 \\ 
                                           &  \team{5} & \train{5} &         4 &         14.94 &         5.49 &         5.70 &        10.14 &         30.70 &         3.75 &  \best{10.27} \\ 
                                           &  \team{3} & \train{3} &         3 &         14.68 & \nbest{5.82} &         5.61 &        10.02 &  \best{25.90} &  \best{3.17} &         17.67 \\ 
                                           &  \team{6} & \train{6} &         5 &         14.03 &         5.06 &         5.65 &         9.98 &         30.40 &         3.80 & \nbest{15.94} \\ 
                                        %   &  \team{9} & \train{9} &         7 &         12.67 &         4.92 &         5.76 &        10.04 &         29.48 &         3.18 &         29.39 \\ 
                                           &  \team{0} & \train{0} &         6 &         12.26 &         4.76 &         6.10 &        10.84 &         33.58 &         4.00 &         18.73 \\ 
                                           &  \team{4} & \train{4} &         7 &         11.56 &         4.55 &         5.61 &         9.79 &         31.16 &         3.60 &         35.30 \\ 
                                           &  \team{7} & \train{7} &         8 &         11.15 &         4.52 &         5.62 & \nbest{9.61} &         31.43 & \nbest{3.17} &         39.06 \\ 
                                           &  \team{8} & \train{8} &         9 &         10.27 &         3.97 &         6.34 &        10.76 &         33.61 &         3.40 &         38.73 \\ 
                                        %   &\team{10} & \train{10} &        11 &          8.42 &         3.41 &         6.52 &        10.91 &         35.61 &         3.42 &         43.22 \\ 
\midrule   
            \multirow{\n}*{\emph{Indoor}}  &  \team{1} & \train{1} &  \best{1} &  \best{33.20} & \nbest{33.12} &  \best{0.70} &         1.63 &  \best{13.08} &  \best{2.89} &         33.52 \\ 
                                           &  \team{3} & \train{3} &         3 & \nbest{33.08} &  \best{33.57} &         0.87 & \nbest{1.35} &         16.52 & \nbest{2.90} & \nbest{21.76} \\ 
                                           &  \team{2} & \train{3} & \nbest{2} &         32.05 &         32.53 & \nbest{0.83} &  \best{1.26} & \nbest{16.00} &         4.11 &         45.68 \\ 
                                        %   &  \team{9} & \train{9} &         7 &         22.55 &         31.29 &         0.85 & \nbest{1.27} &         17.90 &         3.49 &         45.80 \\ 
                                           &  \team{5} & \train{5} &         4 &         22.49 &         29.53 &         1.06 &         1.59 &         23.38 &         4.38 &  \best{14.52} \\ 
                                           &  \team{0} & \train{0} &         6 &         21.11 &         28.96 &         1.04 &         1.51 &         22.77 &         4.60 &         37.09 \\ 
                                        %   & \team{10} & \train{10} &        11 &         20.84 &         29.76 &         1.03 &         1.49 &         21.12 &         5.40 &         78.85 \\ 
                                           &  \team{6} & \train{6} &         5 &         20.25 &         29.52 &         1.03 &         1.48 &         23.37 &         3.96 &         35.68 \\ 
                                           &  \team{7} & \train{7} &         8 &         19.82 &         28.62 &         0.97 &         1.42 &         20.91 &         3.63 &         43.46 \\ 
                                           &  \team{8} & \train{8} &         9 &         19.81 &         28.93 &         1.02 &         1.49 &         21.83 &         5.19 &         69.50 \\ 
                                           &  \team{4} & \train{4} &         7 &         19.18 &         28.34 &         1.09 &         1.61 &         23.24 &         5.14 &         44.02 \\ 
\bottomrule
\end{tabular}

\emph{
\textbf{M}=Monocular -- \textbf{S}=Stereo -- \textbf{D*}=Proxy Depth -- \textbf{D}=Ground-truth Depth
}


==> Tables/syns_cat.tex <==

% SYNS-Patches Category Distribution

% \mycaption{\acl{syns}}{Distribution of images per category in the val/test splits.}

% \begin{tabular}{@{}llllllllll|l@{}}
% \toprule
%                & Agriculture & Indoor & Industry & Misc & Natural & Recreation & Residential & Transport & Woodland & Total \\ 
% \midrule
%   \textbf{Val} &         104 &     67 &       36 &   72 &      36 &         14 &          13 &         4 &       54 &   400 \\ 

%  \textbf{Test} &         211 &     81 &       71 &    0 &     147 &         48 &         110 &        17 &       90 &   775 \\ 
% \midrule
% \textbf{Total} &         315 &    148 &      107 &   72 &     183 &         62 &         123 &        21 &      144 & 1,175 \\ 
% \bottomrule
% \end{tabular}

